Generalized Supergravity Equations and Generalized Fradkin-Tseytlin Counterterm

The generalized Fradkin-Tseytlin counterterm for the (type I) Green-Schwarz superstring is determined for background fields satisfying the generalized supergravity equations (GSE). For this purpose, we revisit the derivation of the GSE based upon the requirement of kappa-symmetry of the superstring action. Lifting the constraint of vanishing bosonic torsion components, we are able to make contact to several different torsion constraints used in the literature. It is argued that a natural geometric interpretation of the GSE vector field that generalizes the dilaton is as the torsion vector, which can combine with the dilatino spinor into the torsion supervector. To find the counterterm, we use old results for the one-loop effective action of the heterotic sigma model. The counterterm is covariant and involves the worldsheet torsion for vanishing curvature, but cannot be constructed as a local functional in terms of the worldsheet metric. It is shown that the Weyl anomaly cancels without imposing any further constraints on the background fields. In the case of ordinary supergravity, it reduces to the Fradkin-Tseytlin counterterm modulo an additional constraint.

==> action.tex <==
\section{Action for the bosonic components}
\label{Ac}

In this section, we will consider the bosonic field equations with the gauge choice \eqref{I:gauge.choice}. For convenience, we shall work in the picture with the Riemannian, torsion-free connection and Riemannian curvature, in which to torsion effects are described by the contorsion tensor. Bars will be dropped throughout.
Setting the fermions to zero and using the gauge \eqref{I:gauge.choice} the field equations \eqref{I:Ricci.torsion.free}--\eqref{I:nab.b.X.trace.torsion.free} read
%
\begin{align}
\label{Ac:Ricci}
	R_{ab} + \frac1{7\kappa} \nabla_{(a} K_{b)} - \frac14 H_{a}{}^{cd} H_{bcd} &=0~,\\
\label{Ac:nab.b.X.asym}	
	\frac2{7\kappa} \nabla_{[a} K_{b]} - \bar{\nabla}^c H_{abc} + \frac1{7\kappa} H_{abc} K^c &= 0~,\\
\label{Ac:nab.b.X.trace}  
	\bar{\nabla}_{a} X^a -2 X_a X^a +\frac12 H^{abc} H_{abc} &= 0~. 
\end{align}

